AuditGPT: Auditing Smart Contracts with ChatGPT

To govern smart contracts running on Ethereum, multiple Ethereum Request for Comment (ERC) standards have been developed, each containing a set of rules to guide the behaviors of smart contracts. Violating the ERC rules could cause serious security issues and financial loss, signifying the importance of verifying smart contracts follow ERCs. Today's practices of such verification are to either manually audit each single contract or use expert-developed, limited-scope program-analysis tools, both of which are far from being effective in identifying ERC rule violations. This paper presents a tool named AuditGPT that leverages large language models (LLMs) to automatically and comprehensively verify ERC rules against smart contracts. To build AuditGPT, we first conduct an empirical study on 222 ERC rules specified in four popular ERCs to understand their content, their security impacts, their specification in natural language, and their implementation in Solidity. Guided by the study, we construct AuditGPT by separating the large, complex auditing process into small, manageable tasks and design prompts specialized for each ERC rule type to enhance LLMs' auditing performance. In the evaluation, AuditGPT successfully pinpoints 418 ERC rule violations and only reports 18 false positives, showcasing its effectiveness and accuracy. Moreover, AuditGPT beats an auditing service provided by security experts in effectiveness, accuracy, and cost, demonstrating its advancement over state-of-the-art smart-contract auditing practices.

==> figures/extract-fn-prompt.tex <==
For the given ERC, List functions in the YAML array with the following format:
  - name: <function name>
    arg_types:
      - name: <parameter name>
        type: <parameter type>
    return_type: <return type, left empty if no return>

ERC:"""
<ERC Documentation>
"""

==> figures/extract-throw-prompt.tex <==
Given an ERC, which contains a list of functions, events, and rules. Each function has its own rules, usually above their Solidity declaration. Rules indicating throw or check usually have patterns like "<subject> MUST throw if <condition>", 
...
 Other patterns that indicate similar meanings also count.
List the conditions in the given ERC for function <function> that need to be thrown or checked in the YAML array with the following format:

<if or unless>: <string, the condition to throw or check>
throw: <boolean, whether it need to throw or should not be thrown>

If no such rule, simply leave it empty.

ERC:"""
<ERC Documentation>
"""


==> figures/fig-extract-fn-prompt.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\scriptsize
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=GPTPrompt,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/extract-fn-prompt.tex}
\mycaption{fig:extract-fn}{LLM prompt template used to extract functions from an ERC}{}
\end{center}
\end{minipage}
\vspace{-0.3in}
\end{figure}
}

==> figures/fig-extract-throw-prompt.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\scriptsize
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=GPTPrompt,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/extract-throw-prompt.tex}
\mycaption{fig:extract-throw}{LLM prompt used to extract throw rules for a function from an ERC}{\textit{(Prompt simplified for illustration purpose.)}}
\end{center}
\end{minipage}
\vspace{-0.3in}
\end{figure}
}

==> figures/fig-fp.tex <==
{
 \begin{figure}[t]

 \begin{minipage}{\columnwidth}
 \begin{center}
 \scriptsize
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=Solidity,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/fp.tex}
 \mycaption{fig:fp}{A false positive.}
{\textit{(Code simplified for illustration purpose.)}
}
\end{center}
\end{minipage}
\vspace{-0.2in}
\end{figure}
}

==> figures/fig-yaml.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\scriptsize
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=YAML,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/yaml.tex}
\mycaption{fig:yaml}{An YAML file contains the result of extracting rules from an ERC}
{\textit{(File simplified for illustration purpose.)}}
\end{center}
\end{minipage}
\vspace{-0.3in}
\end{figure}
}

==> figures/fp.tex <==
contract MyToken {
    string public standard = "Token 0.1";
    string public name;
    string public symbol;
    uint8 public decimals;
    uint256 public totalSupply;

    mapping(address => uint256) public balanceOf;
    mapping(address => mapping(address => uint256)) public allowance;

    event Transfer(address indexed from, address indexed to, uint256 value);

    function transfer(address _to, uint256 _value) {
        ...
    }

    function approve(address _spender, uint256 _value) returns (bool success) {
        ...
    }

    function transferFrom(
        address _from,
        address _to,
        uint256 _value
    ) returns (bool success) {
        ...
    }

    function() {
        throw; // Prevents accidental sending of ether
    }
}


==> figures/yaml.tex <==
erc: 20
functions:
  ...
  - name: transferFrom
    arg_types: 
      - name: _from
        type: address
      ...
    return_type: bool
  ...
events:
  - name: Transfer
    params:
      - name: _from
        type: address
        indexed: true
      ...
  ...
functionRule:
  transferFrom:
    throw:
      - unless: the _from account has deliberately authorized the sender of the message via some mechanism
    return:
      - return whether the transfer is successful
    ...
globalRule:
  check:
    - rule: caller handles or directly returns the result of those calls
      if: call any callee that returns (bool success)
  ...
eventRule:
  Transfer:
    conditions:
      - tokens are transferred, including zero value transfers.
      ...
  ...

==> sections/4_rule.tex <==
\section{Requirement Comprehension}

\subsection{Background.}

\subsection{Experiment setup.} 
In our experiment, we approach the task as a standard machine reading comprehension test. 
Common reading comprehension assessments involve evaluating an individual or system's capability to answer questions based on a provided text. 
As part of this experiment, we create various questions related to ERC requirements and present them to GPT. 
Subsequently, we manually verify each answer provided by GPT against the corresponding ground-truth answer. 
This process allows us to gauge GPT's comprehension and accuracy in addressing the specific ERC-related questions. 

\boldparagraph{Passage.} 
The passage functions as the contextual information from which we extract details to formulate answers for the provided questions. 
In our experiment, we designate the ERC specification as the passage, as shown in \ref{a}. 
Nevertheless, GPT has a restriction on the number of input tokens it can process, with a maximum token limit of 4080. 
Consequently, if the entire specification exceeds this limit, 
we divide it into several smaller chunks that adhere to the token limit. This ensures that each chunk can be processed by GPT effectively. 

\boldparagraph{Question\&Answer.} 
In the evaluation of ERC requirements, we utilize two types of questions: "Yes/No" and "Fact-Based" questions, as depicted in \ref{b}. 
The first "Yes/No" question queries whether the transfer function in ERC20 should emit an event, with the possible responses being "Yes" or "No." 
The purpose of this question is to assess GPT's understanding of a fundamental function requirement—whether a specific action, 
in this case, emitting an event, should be triggered or not. 
The significance of this question type lies in its ability to gauge GPT's grasp of basic function requirements. 
By correctly answering "Yes" or "No," GPT demonstrates its comprehension of whether the transfer function is expected to emit an event as specified in the ERC standard. 
This comprehension is valuable in the context of auditing, as it aids in streamlining the process. 
If GPT understands that a function doesn't need to emit an event, auditing efforts can focus on other aspects without the necessity to verify the emit action, 
saving time and resources during the auditing process. 
Indeed, the "Fact-Based" question in \ref{b} with the corresponding answer in \ref{c} serves a crucial role in improving the accuracy and efficiency of auditing ERC requirements. 
The detailed response in \ref{c} provides the specific event name and elaborates on its attributes or parameters. 
This level of clarity ensures that auditors have accurate information about the expected event emission, enabling them to verify the implementation precisely. 
Having access to the exact event name and its relevant details helps auditors focus their attention on validating the emission of the specific event, 
reducing the chances of overlooking critical aspects during the auditing process. 
With this enhanced comprehension, auditors can efficiently assess whether the transfer function adheres to the ERC requirements concerning event emission. 
Consequently, the auditing process becomes more accurate and streamlined, leading to a higher level of confidence in the smart contract's compliance with ERC standards.

\boldparagraph{Ground-truth.} 
As of our last knowledge, no official centralized repository exists to provide ground-truth answers for ERC requirements. 
Therefore, to establish the ground-truth, we manually review and verify the information from credible sources 
such as the official GitHub repository for Ethereum Improvement Proposals (EIPs), 
which serves as a primary and trustworthy source for ERC specifications. 
Additionally, information can be sought from the official Ethereum Foundation website, Ethereum community forums like Ethereum Stack Exchange and Ethereum's subreddit, 
and relevant research papers related to specific ERCs. When further clarification is needed, 
we communicated with the authors or contributors of specific Ethereum Improvement Proposals to resolve ambiguities. 
We remain updated with the latest developments in the Ethereum ecosystem to ensure the accuracy and reliability of the ground-truth information. 

\begin{enumerate}[label=(\alph*)]
    \item \label{a} \textbf{Passage:} ... 
    Transfers \_value amount of tokens to address \_to, and MUST fire the Transfer event. 
    The function SHOULD throw if the message caller's account balance does not have enough tokens to spend. 
    Note Transfers of 0 values MUST be treated as normal transfers and fire the Transfer event. 
    function transfer(address \_to, uint256 \_value) public returns (bool success) ...
    \item \label{b} \textbf{Question:} Does the transfer function in ERC20 should emit an event? If yes, can you provide guidance on which events should be emitted? 
    \item \label{c} \textbf{Answer:} Yes, according to the ERC20 specification, the transfer function in an ERC20 token contract should emit a Transfer event. 
    The Transfer event should be triggered whenever tokens are transferred, including zero value transfers. 
    The Transfer event has three parameters: \_from (the address tokens are transferred from), \_to (the address tokens are transferred to), 
    and \_value (the amount of tokens being transferred).
\end{enumerate}

\boldparagraph{Metrics.} 
Exact Match (EM) denotes the proportion of questions for which the answer generated by the system perfectly aligns with the ground-truth answer. 
The EM score is calculated as follows, M refers to the count of exact matches, while N represents the total number of questions in the evaluation set:

$$EM=\frac{M}{N}$$

In addition, we also utilize the question-level F1 score as another evaluation metric. 
The F1 score assesses the model's precision and recall in providing answers. It is computed based on the intersection between the system-generated answer and the ground-truth answer. 
By incorporating both EM and F1 score, we gain a comprehensive understanding of the model's performance in Machine Reading Comprehension (MRC) tasks. 

\subsection{Prompts design.} 
The concept behind the designation of prompts is to provide developers with a generic instruction. 
When developers encounter an ERC requirement document, the primary objective is to identify the functions and events that require implementation. 
Therefore, \textbf{\textit{Prompt-1}} is designed to prompt GPT to list all the functions and events mentioned in a given ERC document. 
By using \textbf{\textit{Prompt-1}}, we aim to elicit a comprehensive response from GPT that outlines all the functions and events specified in the ERC document. 
By focusing on listing functions and events, developers can efficiently address the essential aspects of the ERC standard, 
making it easier to meet the required specifications and improve the smart contract's compliance with the ERC guidelines. 
\textbf{\textit{Prompt-2$\sim$7}} are designed to target different ERC requirements, each serving a specific purpose. 
\textbf{\textit{Prompt-2}} focuses on event rules, aiming to extract information about emitted events and the circumstances triggering them. 
\textbf{\textit{Prompt-3}} pertains to checking rules, seeking conditions that cause functions to throw or revert. \textbf{\textit{Prompt-4}} addresses call rules, 
identifying functions to be called when using specific functions. 
\textbf{\textit{Prompt-5}} involves value assignment rules, while \textbf{\textit{Prompt-6}} delves into return rules, 
and \textbf{\textit{Prompt-7}} is dedicated to signature rules. 

\begin{itemize}
    \item \textbf{\textit{Prompt-1}(F+E)}: Can you list all functions/events in ERC[ID]? 
    \item \textbf{\textit{Prompt-2}(RE)}: Does [name] function in ERC[ID] should emit an event? If yes, which events should be emitted?
    \item \textbf{\textit{Prompt-3}(RK)}: Does the [name] function in ERC[ID] revert or throw? If yes, 
    \item \textbf{\textit{Prompt-4}(RC)}: Is there other functions should be called when using [name] function in ERC[ID]?
    \item \textbf{\textit{Prompt-5}(RA)}: If yes, what values should be assigned when calling the [name] function?
    \item \textbf{\textit{Prompt-6}(RR)}: Does [name] function in ERC[ID] have return value? If yes, what is the expected return value when invoking the [name] function? 
    \item \textbf{\textit{Prompt-7}(Total)}: What is the function signature of the [name] function?
  \end{itemize}


\subsection{RQ1: How well does ChatGPT comprehend implementation requirements conveyed in natural language?}

Table~\ref{compre} presents the results obtained by inputting the ERC specification as the passage and using seven prompts for evaluation. 
Almost all prompts achieved a 100\% score on both Exact Match (EM) and F1 metrics, except for prompts related to event rules and checking rules. 
Regarding event rules, GPT exhibited some comprehension limitations, leading to certain misinterpretations. 
For example, it misidentified "isApprovedForSlot" as an "Approved" function, "slotOf" as a changing slot function, and "allowance" as an "approve" function. 
This limitation is likely due to the lack of sufficient description in ERC specifications for these simple functions, such as "isApprovedForSlot" and "slotOf". Consequently, 
GPT attempted to find relevant information for these functions and, in the absence of detailed descriptions, 
it resorted to referencing the descriptions of other functions like "Approved". 
For checking rules,GPT exhibits similar comprehension limitations, such as misinterpreting "isApprovedForAll" as an "Approved" function and "allowance" as an "approve" function. 
While GPT showcases a commendable overall understanding of ERC requirements, 
these limitations are observed primarily with specific "getting" and "checking" methods like "slotOf" and "isApprovedForSlot." 

The impact of these limitations on auditing might be relatively minor. 
Since these methods are primarily used for read operations and validation checks, 
any potential misinterpretations are unlikely to affect the critical functionality or security of smart contracts significantly. 
The read-only nature of "getting" methods ensures that GPT's understanding of these functions would have less influence on the auditing process.
In conclusion, while GPT may have some limitations on certain "getting" and "checking" methods in ERC requirements, 
these limitations are unlikely to have a significant impact on auditing, given the read-only nature of these methods. 
Overall, GPT demonstrates the ability to comprehend ERC requirements effectively, 
and any limitations can be mitigated by providing additional contextual information to enhance its understanding. 

\begin{table}[] \scriptsize
\setlength{\tabcolsep}{3pt} 
\caption{Results of ERC Requirements Comprehension.}\label{compre}
    \begin{tabular}{|l|ll|ll|ll|ll|ll|ll|ll|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}{*}{ERCs}} & \multicolumn{2}{c|}{\textbf{F+E}}                 & \multicolumn{2}{c|}{\textbf{RE}}                  & \multicolumn{2}{c|}{\textbf{RK}}                  & \multicolumn{2}{c|}{\textbf{RC}}                  & \multicolumn{2}{c|}{\textbf{RA}}                  & \multicolumn{2}{c|}{\textbf{RR}}                  & \multicolumn{2}{c|}{\textbf{Total}}               \\ \cline{2-15} 
    \multicolumn{1}{|c|}{}                      & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{F1} \\ \hline
    ERC20                                       & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   &                      & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   & 1.0                        \\ \hline
    ERC721                                      & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   &                      & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   &  1.0                       \\ \hline
    ERC777                                      & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   &                      & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   &  1.0                       \\ \hline
    ERC3525                                     & \multicolumn{1}{l|}{1.0}   & 1.0                & \multicolumn{1}{l|}{0.64}  & 0.66                 & \multicolumn{1}{l|}{}   &                         & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{}   &                         \\ \hline
    \textbf{All}                                & \multicolumn{1}{l|}{1.0}   & 1.0                & \multicolumn{1}{l|}{0.90}   & 0.96                & \multicolumn{1}{l|}{}   &                         & \multicolumn{1}{l|}{1.0}   &  1.0                 & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{1.0}   & 1.0                  & \multicolumn{1}{l|}{}   &                         \\ \hline
    \end{tabular}
    \end{table}


\label{sec:understanding}


==> sections/5_prompt.tex <==

\section{Prompt Design}




% To answer RQ1, use XXX metrics
% => setting, exp, result
% dataset (TODO)
% differnet prompt has big effect on the response
% exp5 and exp6 can be reported together


% exp10 => handle how many # of errors in the code
% => code complexity

We aim to build an auditing tool using ChatGPT, 
which can inspect whether a smart contract adheres to the requirements specified 
in the corresponding ERC description. 
Considering this specific task, we break down each prompt into three components:
1) ERC requirements in natural language, 2) Solidity code for ChatGPT to examine, 
and 3) textual instructions that explain the task. 
%As the chosen contracts do not contain many implementation errors that violate ERC requirements, we modify the contracts to introduce violations for the purpose of our experiments. 
%This section first explains the process of injecting ERC requirement violations. 
This section discusses how to construct the three components 
to ensure ChatGPT performs well in auditing. 




\subsection{ERC Requirement Settings}
\label{sec:requirement}

\input{tables/tbl-requirement}

As discussed in Section~\ref{sec:meth}, the training set of ChatGPT
includes ERC-20, ERC-721, and ERC777. 
Consequently, the first question we 
explore is whether it is necessary to include the requirements in these ERCs when constructing prompts. 
Since there is a strict limit of 4097 tokens for each prompt, by simplifying the requirement part, we can allocate more space for the code and instruction parts. 
Moreover, 
ChatGPT does not know ERC3525, and given its length exceeds the prompt limit, 
we need to devise a method to input ERC3525 for ChatGPT to audit ERC3525 contracts. 



%We design three experiments to examine whether 
%requirement descriptions in ERC20, ERC721, and ERC777 are necessary for
%ChatGPT to audit the corresponding contracts. 
%The instruction is "Given an ERC20 specification and a solidity code.
%The function transfer might have errors like missing emitting required events.
%Check whether the function transfer emits events required by the ERC20 specification correctly?". The instruction might not be the most effective one since we have not yet conducted experiments about instruction. It is used simply for comparing the ChatGPT capability of auditing with or without specification.

\italicparagraph{Known ERCs.}


We design \textit{Experiment-1} to explore whether we 
still need to provide requirements in ERC20, ERC721, and ERC777 
in prompts for ChatGPT to audit the corresponding contracts.

For \textit{setting-1}, we construct one prompt for each contract, 
with the complete ERC description as the requirement component and the entire contract as 
the code part. We require ChatGPT
to examine whether the contract is compliant with the ERC.
\textit{Setting-2} is the same as the first one, except that we omit the requirement part. 
These two settings simulate the scenario where a programmer 
relies on ChatGPT to examine an entire contract.

\input{snippets/inj-emit-err}

For the remaining three settings, our focus shifts to the token-transfer function 
in each contract. Those
functions are required to emit an event following a transfer action by the ERCs. {\color{red} As shown in the Listing \ref{lst:rm-emit},}  we remove 
the emit instruction for each function to inject an error in the function.
We use the token-transfer function (without anything outside the function scope)
as the code part. We require ChatGPT to inspect whether 
the function fails to emit any event required by the ERC to
simulate the situation where ChatGPT solely inspects a function body for auditing purposes. 
The three settings differ from each other in the requirement part. 
We use the complete ERC description as the requirement part for \textit{setting-3}, 
ignore the requirement part for \textit{setting-4}, 
and only use the descriptions of the token-transfer functions in the ERCs for \textit{setting-5}. 

{\color{red} For ERC20, the description of the token-transfer function is indeed the requirement of the function, a paragraph on top of the function signature. 
However, in ERC721 and ERC777, the requirements are grouped by functionality in the specification. The requirements of either emitting events or sending tokens are far from the description of the function. We treat the requirements of sending tokens and related event emissions as part of the description of the token transfer function and put them into the prompt for \textit{setting-5} after grouping them manually.

For \textit{setting-1} and \textit{setting-2}, the results cannot lead to any conclusion: 1) ChatGPT does not identify the two violations in the ERC20 contract. 2) The requirements of ERC721 and ERC777 are too long to fit into the prompt. This also affects them in \textit{setting-3} but is mitigated by \textit{setting-5}.
For \textit{setting-3}, \textit{setting-4} and \textit{setting-5}, ChatGPT successfully identified all three manually injected violations about missing required event emission with and without the requirements. 
The results show that ChatGPT can audit the contract without explicitly mentioning the requirements in the prompt if it "learns" the requirements before (a.k.a, in the model's training set). 
}



\subsection{Solidity Code Settings}

\input{tables/tbl-code}

We conduct \textit{Experiment-3} to investigate the proper way of inputting code
to ChatGPT. This is necessary because many contracts exceed ChatGPT’s token limit 
and cannot be directly used as the code part. Furthermore, including unnecessary information 
in the input may divert ChatGPT’s focus and reduce its detection accuracy. 

We create two variations for each contract, with one error injected in each variation.
When creating a prompt, we focus on one variation.  
As what we did in Section~\ref{sec:requirement}, we delete the event-emit 
instruction in the token transfer function to create the first variation.
For the second variation,  
we select the {\color{red}authorizing} function in each contract. 
As all the ERCs mandate the {\color{red}authorizing} function to 
throw an exception when a specific condition is not met, 
we remove the source code lines responsible for throwing the exception and 
checking the condition.  

We explore four different settings in this experiment with progressively 
less code used as the code part for the latter settings. 
In \textit{setting-1}, we use the complete contract as the code component. 
For the other three settings, our focus narrows down to the function with the injected error. 
In \textit{setting-2}, we input not only the function and also 
all program elements beyond the function
that are used by it, including the function’s callees, the declarations of the contracts 
containing the function and its callees, and all contract fields used by the function. 
In \textit{setting-3}, we use the function, its callees, and the declarations of the related contracts, 
since we observe that sometimes a function and an event
share the same name, which may confuse ChatGPT.
Lastly, in \textit{setting-4}, we only input the function with the injected error, without anything 
outside the function, the same as what we did in Section~\ref{sec:requirement}. 

We ignore the requirement part for ERC20, ERC721, and ERC777 contracts, and {\color{red} adding the function level requirements for the ERC3525}.

For instructions, {\color{red}we choose a working one but might be the best since we have not conducted the instruction experiments yet.

As shown in Table \ref{tab:exp-3}, \textit{setting-1}, putting full contract code in the prompt has the worst result.  For \textit{setting-4}, although it does have many true positives, it is impractical to use it in reality since most of the large Solidity implementations will separate the complex transferring token logic into multiple functions. ChatGPT cannot audit the function by merely function calls without their implementation detail. For the last two settings, the results of \textit{setting-3} are better than the \textit{setting-2} with much more true positives. This is due to \textit{setting-3} omitting the texts that are either  unrelated to the violations or misleading. For example, the event declaration can mislead the ChatGPT to answer "the given contract indeed emits the event". The false positives, after analyzing the responses, are related to the "check" rule. One function usually has only one or two event emission requirements but can easily have more than five or more "check" rules. A vague instruction in the prompt will lead to an imprecise answer from ChatGPT. We will explore this more in the next section.
}




\subsection{Textual Instruction Settings}
We design three experiments to examine how textual instruction affects ChatGPT to audit the corresponding contracts.

\input{tables/tbl-instruction-part1}

\input{snippets/exp-inst-st1}

In \textit{setting-1}, we construct the prompt with the instruction "whether the function <name> is compliant with the <ERC> specification", as shown in the Listing \ref{lst:exp-inst-st1}. In the ideal scenario, we want the ChatGPT to find out all inconsistencies by merely providing simple instructions in the prompt.

{
    \color{red} The results of \textit{setting-1} show that ChatGPT does not really understand what is the meaning of compliance. From a contract auditing perspective, the compliance infers following every rule specified in the ERC specification. Clearly, ChatGPT does not have the same definition of compliance as our understanding. We need to provide clearer instructions to guide ChatGPT to audit.
}

\input{snippets/exp-inst-st2}

In \textit{setting-2}, we construct the prompt with the clear auditing target, as shown in Listing \ref{lst:exp-inst-st2}, to check whether the function violates a specific type of rule in the specification. Unlike the \textit{setting-1}, which requests ChatGPT to audit the contract in one sentence, \textit{setting-2} breaks the whole auditing task into auditing six types of rules individually. 

{  \color{red}
    Compared to the \textit{setting-1}, \textit{setting-2} provides a clearer auditing target for ChatGPT.
    The results of \textit{setting-2} show ChatGPT can find three "event" rule violations on the ERC20 contracts. 
    It is better than the \textit{setting-1} but still has much room to improve. After reviewing the responses containing false positives and false negatives, we noticed that the response usually will try to follow the intent of the prompt. "Whether function emits" and "Whether function throws" implicitly hint at ChatGPT to generate a "yes", which is opposed to a contract auditing tool.
    \textit{setting-3} is designed to utilize this pattern.
}

\input{snippets/exp-inst-st3}

In \textit{setting-3}, we construct the prompt with the opposite inclination  in \textit{setting-2}, as shown in the Listing \ref{lst:exp-inst-st3} to check whether the function has a specific type of rule violation. 

{  \color{red}
The results of \textit{setting-3} confirm that we successfully utilized this pattern. 
ChatGPT finds many more true positives in the ERC20 and ERC777.
But the zero true positives on ERC721 still have no improvements compared to the previous settings.
Reviewing the results from the previous settings, the quality of response from ChatGPT improves as more precise instruction is given. Maybe ChatGPT cannot identify the violation because the instruction is not precise enough. For example, for auditing the "check" rule, instead of using the word "throw", maybe "check" is a more general word for ChatGPT to understand, since other programming languages might have different names for the "throw" mechanism. Same thing for the "event" rule, instead of using "emitting event", "event emission" might be a more understandable word for ChatGPT. \textit{setting-4} is designed to verify the effectiveness of the wording used to describe the violation.

}

\input{snippets/exp-inst-st4}

In \textit{setting-4}, we maintain the inclination used in \textit{setting-3} but instead use some different words closer to people's common sense or what ChatGPT used in its responses to describe the error, as shown in the Listing \ref{lst:exp-inst-st4}.

{  \color{red}
The results turn out that not only the inclination, the error-descriptive words can also profoundly impact the quality of the ChatGPT response. From Table \ref{tab:exp-4p1}, \textit{setting-4} has the most true positives and least false positives and false negatives. However, the all experiment settings in  Table \ref{tab:exp-4p1} only cover the situation that the error we ask ChatGPT to check is aligned with the actual error in the code. In real world scenario, the users do not have such information without auditing the contract.
}


\input{tables/tbl-instruction-part2}

\subsection{Real World Scenario}
{  \color{red}
The current SOTA instruction has a strong inclination to induce ChatGPT replies with confirmed violations. In a real-world scenario, we do not know what exactly the violations the code has and how many are they.  We want to see whether this instruction works on code without violation and with other types of violation not in the scope of instruction. We also want to know, instead of asking ChatGPT to audit six times for six types of violations, if it is possible to put all six instructions into one prompt to simplify the auditing process.

We will manually inject all six types of rule violations into token-transfer functions from ERC20, ERC721 and ERC777 that have the corresponding rules required in their ERCs. Each type of violation will be injected into three different contract functions and each of them is from different ERCs to cover the diversity. The token-transfer function in ERC20 does not have a "call" rule and "assign rule". The token-transfer function in ERC721 and ERC777 do not have a "return" rule since they do not have a return value. The token-transfer function in ERC721 does not have an "assign" rule.

As shown in Table \ref{tab:exp-4p2}, we can see that although asking ChatGPT in a negative way can find many true positives, it also brings many false positives when the error asked to ChatGPT is different from the actual error in code. A reasonable conclusion is ChatGPT will try its best to follow your inclination in the prompt and generate the result. If the prompt has a strong inclination, the response from ChatGPT will most likely follow the way. Another reason to cause many false positives is the vague question. When a function has many checks mentioned in the specification, asking ChatGPT like "missing any check" is not precise enough for ChatGPT to find out the correct missing one. It either will response 
they all exist or none of them exist. The reason for false negatives from "signature" and "assign" are similar, the description of the errors is too general. A valid signature infers the correct function name, correct parameter types, and correct return types. ChatGPT need to infer these rules from a simple sentence "whether the function has the incorrect signature", which will increase the false negatives.

\input{snippets/exp-inst-detail-ask-event}

Clearly, we need to avoid asking negatively and increase the precision of the error description in the instruction to reduce false positives and false negatives. As Listing \ref{lst:exp-inst-detail-ask-event} shown, the instruction includes the specific event name instead of "any" in previous settings. Notices that there is an extra "and all its
callees" after the function name, this is because ChatGPT sometime only checks the scope of the target function "transfer", not including its callees. Without including this note, ChatGPT will have many false positives. Including this note in the instruction clarifies our asking and reduces the potential false positives.


\input{tables/tbl-instruction-part3}

As shown in Table \ref{tab:exp-4p3}, after changing the instruction to explicit asking style, the number of false positives dramatically reduced. 

 }

\if 0

\subsection{Prompt Settings }
In order to answer the research questions mentioned earlier, two kinds of information are necessary: the instruction (what the GPT model should do), and context (specification and code).
The prompt sent to the GPT model can be roughly divided into the following three parts:
\begin{enumerate}
    \item Instruction
    \item Specification
    \item Code
\end{enumerate}

And each part has the following different choices:

\subsubsection{Instruction}
\begin{enumerate}
    \item General asking for the whole code/contract
    \item General asking for a single function
    \item Specific asking a violation type for the whole code/contract
    \item Specific asking a violation type for a function
    \item Specific asking a violation type for a function + hint 
\end{enumerate}
\subsubsection{Specification}
\begin{enumerate}
    \item Full spec
    \item No spec
\end{enumerate}
\subsubsection{Code}
\begin{enumerate}
    \item Full code
    \item Target function and its callees
    \item Target function, its callees, and their contract declaration
    \item Interface only
\end{enumerate}


This list contains all the combinations of parts we used in the later experiments.


\subsubsection{ Setting 1 }
Instruction(General Asking for code) + Specification(Full) + Code(Full)

Example Prompts: 
\begin{enumerate}
\item "Whether the code is compliant with the specification" + <full specification> + <full code>
\item "Find out any consistency between the code and specification" + <full specification> + <full code>
\end{enumerate}

\subsubsection{ Setting 2 }
Instruction(General Asking for code) + Code(Full)

Example Prompts: 
\begin{enumerate}
\item Whether the code is compliant with the specification + <full code>
\item Find out any consistency between the code and specification  + <full code>
\end{enumerate}

\subsubsection{ Setting 3 }
Instruction(General Asking for a function) + Code(function and its callees)

\begin{enumerate}
\item "Whether the function is compliant with the specification" + <target function and its callees>
\end{enumerate}


\subsubsection{ Setting 4 }
Instruction(Specific Asking for a function) + Code(function and its callees)

\begin{enumerate}
\item "Whether the function miss any required event" + <target function and its callees>
\end{enumerate}

\subsubsection{ Setting 5 }
Instruction(Specific asking a violation type for a function + hint ) + Code(function and its callee + Contract Decl)
\begin{enumerate}
\item "The function might contain errors like XXX, whether the function has XXX" + <target function and its callees>
\end{enumerate}

\subsubsection{ Setting 6 }
TODO
\subsubsection{ Setting 7 }
TODO
\subsubsection{ Setting 8 }
TODO


\subsection{ Experiment Settings and Results }
In order to comprehensively evaluate the GPT capabilities in various environments, multiple different environment settings are necessary to be conducted. Each experiment might involve one or more different prompt settings regarding different findings or purposes. Some scenarios might require some violations or even some specific violations present in the code. Due to the dataset limitation, some violations are injected into the code if the code does not have corresponding violations.


\subsubsection{ Experiment 1: Naive try }
In the beginning, we hope the GPT model identifies all the violations with context information as much as  possible in order to find out every inconsistency between the specification and the code.
We start with the prompt with the full context information: complete specification and code, which is prompt setting 1.

This experiment runs on all 3 ERC20 contracts since all the other contracts exceed the GPT model limitation. 
Every contract contains at least one violation.

\subsubsection{ Experiment 1 result }
The GPT model cannot find any violation in the code. 
After analyzing the violation, we found that each violation actually is only highly related to a few sentences regarding all the context information in the prompt: a sentence of rule in the context and a few sentences of the Solidity code. 
It is intuitive to make a guess that the GPT model cannot find out any violations due to massive unrelated information.
There are several possible places that can be improved: 1. Specification is too long 2. The code is too long.
We can start with the specification part.

\subsubsection{ Experiment 2: Does specification must present if it is in the GPT model's training set? }
Due to the design of the LLM model, a model will remember much information from its training set. Since the GPT model 3.5 used almost all the internet information before Sept. 2021, it is highly possible that it already learned many popular specifications in its training set. The specification usually consumes a large number of tokens in the prompt. It might either block the space for putting a large contract with long code in the prompt or might distract the GPT's attention. 

This experiment runs on all 3 ERC20 contracts with prompt setting 2 to see whether GPT can give an equal or better response compared to setting 1.


\subsubsection{ Experiment 2 result}
The GPT model still cannot find any violation in the code.
% Although the GPT model cannot find any issue, considering the response and other experiments about ERC understanding, we confirmed that the GPT model has a memory of the popular ERCs. 
% But whether we can find out inconsistencies without mentioning the spec in the prompt need to be further confirmed

\subsubsection{ Experiment 3: Does code length matter? }
Experiment 3 intends to let the GPT model find a violation for a specific function.
For ERC20, we choose one of the most important functions "transfer" as our target function.
Each function is injected with all 5 different violations.
The prompt setting 3 is used in this experiment. 

\subsubsection{ Experiment 3 result }
The GPT model still cannot find any violation in the code.

\input{tables/exp4_table}

\subsubsection{ Experiment 4: Does instruction matter? }
The prompt setting 4 is used in this experiment.

\subsubsection{ Experiment 4 result }
The GPT model can find some violations in the code. But there are still many violations that cannot be found.

\input{tables/exp5_table}
\subsubsection{ Experiment 5: Does add "hint" in the instruction help? }
% TODO

\subsubsection{ Experiment 5 result}
Yes
%TODO

\subsubsection{ Experiment 6: Does "hint" cause false positive? }
\subsubsection{ Experiment 6 result }
No
\subsubsection{ Experiment 7: Does "additional rule" help reduce the false positives and false negatives? }
\subsubsection{ Experiment 7 result }
No

\subsubsection{ Experiment 8: Does current SOTA instruction have false positive on code without error or with out-of-scope error  }
\subsubsection{ Experiment 8 result }
Around 18\% for ERC20 3 contracts 61 tries

\subsubsection{ Experiment 9: Can the GPT model handle obfuscation }
\subsubsection{ Experiment 9 result }
\begin{enumerate}
\item Good at mangled variable names.
\item Can identify simple logic conditions like "if(true){...}", "while(cond){ ...;cond = false;}"
\item Combined with previous experiment (4,5,6,7), the GPT cannot handle complex logic like "if(a == b \&\& c == d \&\& e == f)"
\item Combined with previous experiments (4,5,6,7), the GPT can handle the required action in other functions with long distance of call graph or control flow graph.
\end{enumerate}

\subsubsection{ Experiment 10: Can the GPT support finding multiple violation types using current SOTA instruction? }
\subsubsection{ Experiment 10 result }
No. It is better to use 1 violation type at a time.

\subsubsection{ Experiment 11: Can SOTA be used for whole code }
Since the GPT model can handle fairly long code(from experiment 9), combined with the previous conclusion from experiment 3 that code length matters, it is better to say content in the code matters. 
In order to verify the SOTA cannot be used for the whole code and the necessity of slicing the whole Solidity contract into functions, the SOTA instruction is used with the full code.
\subsubsection{ Experiment 11 result }
No.


\subsection{ Findings }

\begin{enumerate}

    \item The GPT model can find XXX, XXX, XXX violation types on XXX conditions

    Experiment 4,5,6,7
    
    \item The GPT model can find violations without including specifications in the prompt if it is in the training set

    Experiment 2
    
    % TODO: what is the meaning of simple
    \item The GPT model cannot handle the complex logic conditions

    Experiment 4,5,6,7,9
    
    % TODO: what is the meaning of complex
    \item The GPT model can handle mangled variable names

    Experiment 9
    
    \item The GPT model can handle long(cannot longer its token limitation) Solidity code after "slicing"

    Experiment 9

    \item The GPT model will 100\% trust what you provide in the prompt. It is critical to point out the code might contain errors.

    Experiment 5
    
    \item The GPT model can reduce FP/FN by providing the fine-grained description in the first or following prompt

    Experiment 7
    
    \item The GPT model will have more FN/FP as more violation types you ask it to check.

    Experiment 10

    \item The GPT model cannot identify violation type if many related  words existed
     % need to clarify here what is related (for example, missing XXX but interface has XXX)
     
    
\end{enumerate}

\fi








==> sections/6_exp3.tex <==
\section{Complex Code Handling}

\subsection{Requirement Violation Injection}
There are various ways that can cause the same violation type.
We manually concluded the following common root causes that can trigger such violations. 
For the 3 violations related to missing action, they can share the same group of root causes.

When evaluating the GPT model, it usually requires the code in the prompt to have a certain number or types of violations in order to test the capabilities of the GPT model.
However, due to the limitation of the dataset, not all of them has the corresponding violations required by the experiment design.
We will inject corresponding violations depending on the experiments' need if the original Solidity code does not have such violations.
For each of the root causes, fine-grained rules are provided to be used as violation injection methods.

% \input{tables/vio_inj_table} too ugly

\begin{enumerate}
    \item Missing required action
    \begin{enumerate}
        \item Incorrect action
            \begin{enumerate}
                \item No action
                \item Another action
            \end{enumerate}
        \item Incorrect parameter(s)
            \begin{enumerate}
                \item Wrong order
                \item Wrong value
            \end{enumerate}
        \item Incorrect condition(s)
            \begin{enumerate}
                \item No condition(s)
                \item Wrap action with if(false){ ... }
                \item condition(s) \&\& false != false
                \item condition(s) \&\& true != true
                \item !condition(s)
                \item Wrap action with while(false){ ... }
                \item conditions(s) \&\& (true != true || 1 != 1)
            \end{enumerate}
    \end{enumerate}
    \item Incorrect function signature
    \begin{enumerate}
        \item Missing function signature(s)
        \item Incorrect name
        \item Incorrect number of  parameter(s)
        \item Incorrect parameter type(s)
        \item Incorrect return type
    \end{enumerate}
    \item Incorrect function return value
\end{enumerate}

\subsection{Obfuscation}
In order to test the Solidity code complexity boundary that the GPT model can audit, the following obfuscation methods are used in the experiments.

{\color{red} mangled variable names }

{\color{red} complex logic conditions }

{\color{red} long control flow distance }

{\color{red} long control inter-procedural distance }




% \begin{enumerate}
%     \item Mangling function local variable \& parameters
%     \item Wrap required condition with while(cond) { <required action>; cond = false; }
%     \item Wrap required condition with if(true) { <required action> }
%     \item Create a separate function X to wrap <required action> and replace original <target code> with X()
%     \item Insert code between the condition and <required action>

% \end{enumerate}

==> sections/8_related.tex <==
\section{Related Work}



\section{Conclusion}

==> snippets/erc1155-high.tex <==
\begin{lstlisting}[label={lst:erc1155-high},captionpos=b, caption={ERC1155 Contract 0x6482e7f6: high violation severity found by AuditGPT},language=solidity]
function safeTransferFrom(address from, address to, uint256 id, uint256 value, bytes memory data) public {
    _update(from, to, id, value);
}

function _update(address from, address to, uint256 id, uint256 value) internal {
    if (from != address(0)) {
        _balances[id][from] -= value;
    }
    if (to != address(0)) {
        _balances[id][to] += value;
    }
}
\end{lstlisting}

==> snippets/erc20-high.tex <==
\begin{lstlisting}[label={lst:erc20-high},captionpos=b, caption={ERC20 Contract 0x294d7be2: high violation severity found by AuditGPT},language=solidity]
function transferFrom(
    address from,
    address to,
    uint256 amount
) public virtual override returns (bool) {
    _transfer(from, to, amount);
    return true;
}

function _transfer(
    address from,
    address to,
    uint256 amount
) internal virtual {
    require(from != address(0), "ERC20: transfer from the zero address");
    require(to != address(0), "ERC20: transfer to the zero address");
    uint256 fromBalance = _balances[from];
    require(
        fromBalance >= amount,
        "ERC20: transfer amount exceeds balance"
    );
    unchecked {
        _balances[from] = fromBalance - amount;
        _balances[to] += amount;
    }
    emit Transfer(from, to, amount);
}
\end{lstlisting}

==> snippets/exp-inst-detail-ask-event.tex <==
\begin{lstlisting}[label={lst:exp-inst-detail-ask-event},captionpos=b, caption={Example of prompt in instruction experiment explicitly asking event emission},language=GPTPrompt]
Given the solidity code for ERC20 specification.
Check whether the function transfer(and all its callees) emits the "Transfer" event required by the ERC<erc> specification?

code:"""
<code>
"""
\end{lstlisting}

==> snippets/exp-inst-st1.tex <==
\begin{lstlisting}[label={lst:exp-inst-st1},captionpos=b, caption={Example of prompt in instruction experiment setting-1},language=GPTPrompt]
Given the solidity code for ERC20 specification.
Check whether the function transfer is compliant with the ERC20 specification?

code:"""
<Solidity code>
"""
\end{lstlisting}

==> snippets/exp-inst-st2.tex <==

\begin{lstlisting}[label={lst:exp-inst-st2},captionpos=b, caption={Example of prompt in instruction experiment setting-2},language=GPTPrompt]
Given the solidity code for ERC20 specification.
Check whether the function transfer emits required events required by the ERC20 specification?

code:"""
<Solidity code>
"""
\end{lstlisting}

==> snippets/exp-inst-st3.tex <==
\begin{lstlisting}[label={lst:exp-inst-st3},captionpos=b, caption={Example of prompt in instruction experiment setting-3},language=GPTPrompt]
Given the solidity code for ERC20 specification.
Check whether the function transfer is missing emitting any events required by the ERC20 specification?

code:"""
<Solidity code>
"""
\end{lstlisting}

==> snippets/exp-inst-st4.tex <==
\begin{lstlisting}[label={lst:exp-inst-st4},captionpos=b, caption={Example of prompt in instruction experiment setting-4},language=GPTPrompt]
Given the solidity code for ERC20 specification.
Check whether the function transfer is missing any event emissions required by the ERC20 specification?

code:"""
<Solidity code>
"""
\end{lstlisting}

==> snippets/inj-emit-err.tex <==


\begin{lstlisting}[label={lst:rm-emit},language=Solidity,captionpos=b, caption={Transfers \_value amount of tokens to address \_to, and MUST fire the Transfer event}]
function transfer(address _to, uint256 _value) public returns (bool) {
    require(_to != address(0));
    require(_value <= balances[msg.sender]);
    // SafeMath.sub will throw if there is not enough balance.
    balances[msg.sender] = balances[msg.sender].sub(_value);
    balances[_to] = balances[_to].add(_value);
-   emit Transfer(msg.sender, _to, _value);
    return true;
}

\end{lstlisting}

==> tables/tbl-code.tex <==

\begin{table}

\centering
\small
  \mycaption{tab:exp-3}
{Results of \textit{Experiment-3}.}
{\textit{(Contract: contract code, Sliced: function and its sliced code, 
    and Fn+Callees: function, its callees, 
    and the declarations of the contracts containing the functions.
TP: true positives, FP: false positives, and FN: false negatives.}
}
{
\resizebox{\columnwidth}{!}{
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
     \multirow{2}{*}{\textbf{ERC}} & \multicolumn{3}{c|}{\textbf{Contract}} & \multicolumn{3}{c|}{\textbf{Sliced}} & \multicolumn{3}{c|}{\textbf{Fn+Callees}} & \multicolumn{3}{c|}{\textbf{Fn}} \\
     \cline{2-4}
     \cline{5-7}
     \cline{8-10}
     \cline{11-13}
     & TP & FP & FN & TP & FP & FN & TP & FP & FN & TP & FP & FN \\
     \hline
      20  & 3 & 0 & 7 & 2 & 0 & 4 & 6 & 1 & 0 & 6 & 1 & 0     \\ 
      \hline 
      721 & 0 & 0 & 6 & 0 & 0 & 6 & 0 & 0 & 6 &  0 & 3 & 3   \\                                                        \hline
      777 & 0 & 0 & 6 & 3 & 0 & 3 & 5 & 3 & 1 &  2 & 3 & 1  \\                                                        \hline
      3525 & 0 & 0 & 6 & 0 & 0 & 6 & 3 & 0 & 3 & 3 & 0  & 3\\ 
      \hline

  %\bottomrule
  \hline
  \end{tabular}

  }
}

\end{table}


% ERC721 &  $(0,0,6)$ & $(0,0,6)$ & $(0,0,6)$ & $(0,3,3)$  \\                                                        \hline
%       ERC777 & $(0,0,6)$ & $(3,0,3)$  & $(5,3,1)$ & $(2,3,1)$  \\                                                        \hline
%       ERC3525 & xxx & xxx & xxx & xxx \\ \hline 

==> tables/tbl-ercs.tex <==
\begin{table}
\centering
\small
  \mycaption{tab:ercs}
{Table of \textit{Studied ERCs}.}
{\textit{(F: the number of functions, E: the number of events, RE: the number of event rules, RK: the number of checking rules, RC: the number of call rules, RA: the number of assignment rule, RR: the number of return rules, Total: the sum of rules mentioned above and the number of signature rules(F+E) )}}
{
  \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
    \hline
        & \textbf{F} & \textbf{E} &  \textbf{RE} & \textbf{RK} & \textbf{RC} & \textbf{RA} & \textbf{RR} & \textbf{Total} \\
     \hline
      ERC20  & 9 & 2  & 7 & 5 & 0  & 0 & 9 & 32    \\ \hline 
      ERC721 & 17 & 3  & 7 & 30 & 3  & 1 & 12 & 73     \\                                                        \hline
      ERC777 & 13 & 5  & 32 & 36 & 44  & 26 & 8 & 164     \\                                                        \hline
      ERC3525 &  14 & 4 & 16 & 48 & 2  & 3 & 11 & 98   \\ \hline 

  %\bottomrule
  \hline
  \end{tabular}
}
\end{table}

==> tables/tbl-human.tex <==
\begin{table}[h]
\centering
\begin{tabularx}{\columnwidth}{lcccccc}
\hline
\textbf{Metric} & \textbf{TP} & \textbf{FP} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
\hline
Human           & 84          & 1           & 35          & 98.82\%            & 70.59\%         & 82.35\%           \\
Tool            & 117         & 0           & 2           & 100.00\%           & 98.32\%         & 99.15\%           \\
\hline
\end{tabularx}
\caption{Performance Comparison: Human vs. Tool}
\label{tab:performance_correct}
\end{table}

==> tables/tbl-instruction-part1.tex <==
\begin{table}
\centering
\small
  \mycaption{tab:exp-4p1}
{Results of \textit{Experiment-4 Part 1}.}
{\textit{(General: whether function is compliant, Positive: whether function has required action, Negative: whether function is missing required action(i.e, emitting event), and Negative*: whether function is missing required action(i.e, event emission).
TP: true positives, FP: false positives, and FN: false negatives.)}
}
{
  % \begin{tabular}{|l|c|c|c|c|}
  %   \hline
  %               & \textbf{General} & \textbf{Correct} &  \textbf{Missing} & \textbf{Missing2}   \\
  %    \hline
  %     ERC20  &  $(0,0,6)$ & $(3,4,3)$  & $(6,0,0)$ & $(6,0,0)$     \\ \hline 
  %     ERC721 &  $(0,0,6)$ & $(0,0,6)$ & $(0,0,6)$  & $(3,1,3)$  \\                                                        \hline
  %     ERC777 & $(0,0,6)$ & $(0,3,6)$  & $(4,5,2)$ & $(6,0,0)$  \\                                                        \hline
  %     ERC3525 & xxx & xxx & xxx & xxx  \\ \hline 
\resizebox{\columnwidth}{!}{
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
     \multirow{2}{*}{\textbf{ERC}} & \multicolumn{3}{c|}{\textbf{General}} & \multicolumn{3}{c|}{\textbf{Positive}} & \multicolumn{3}{c|}{\textbf{Negative}} & \multicolumn{3}{c|}{\textbf{Negative*}} \\
     \cline{2-4}
     \cline{5-7}
     \cline{8-10}
     \cline{11-13}
     & TP & FP & FN & TP & FP & FN & TP & FP & FN & TP & FP & FN \\
     \hline
      20  & 0 & 0 & 6 & 3 & 4 & 3 & 6 & 0 & 0 & 6 & 0 & 0     \\ 
      \hline
      721  & 0 & 0 & 6 & 0 & 0 & 6 & 0 & 0 & 6 & 3 & 1 & 3     \\ 
      \hline
      777  & 0 & 0 & 6 & 0 & 3 & 6 & 4 & 5 & 2 & 6 & 0 & 0     \\
      \hline
      3525  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0     \\

  \hline
  \end{tabular}
  }
}
\end{table}

==> tables/tbl-instruction-part2.tex <==
\begin{table}
\centering
\small
  \mycaption{tab:exp-4p2}
{Results of \textit{Experiment-4 Part 2}.}
{\textit{$(x, y, z)$: $x$ true positives, $y$ false positives, and $z$ false negatives.)}
}
{
\resizebox{\columnwidth}{!}{
  \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
          \backslashbox{Ask}{Actual}
      & \textbf{Event} & \textbf{Check} &  \textbf{Call} & 
                \textbf{Assign} &
                \textbf{Signature} & \textbf{Return}  \\
     \hline
      \textbf{Event}  &  $(3,0,0)$ & $(0,2,3)$  & $(0,2,2)$ & $(0,1,1)$ & $(0,3,3)$ & $(1,0,0)$  \\ 
      \hline 
      \textbf{Check}&  $(0,5,0)$ & $(2,4,1)$  & $(1,3,1)$ & $(0,1,1)$ & $(0,5,3)$ & $(1,0,0)$\\                                                        \hline
       \textbf{Call} &  $(0,0,3)$ & $(0,1,3)$  & $(1,1,1)$ & $(0,0,1)$ & $(0,1,3)$ & $(0,1,1)$ \\                                                        \hline
       \textbf{Assign} &  $(0,0,3)$ & $(0,0,3)$  & $(0,0,2)$ & $(0,0,1)$ & $(0,0,3)$ & $(0,0,1)$ \\                                                        \hline
      \textbf{Signature} &  $(0,0,3)$ & $(0,0,3)$  & $(0,0,2)$ & $(0,0,1)$ & $(1,0,2)$ & $(0,0,1)$ \\ 
      \hline 
      \textbf{Return} &  $(0,0,3)$ & $(0,0,3)$  & $(0,0,2)$ & $(0,0,1)$ & $(0,0,3)$ & $(1,0,0)$ \\ 
      \hline
      \textbf{All} &  $(3,4,0)$ & $(1,4,2)$  & $(0,5,2)$ & $(0,3,1)$ & $(0,5,3)$ & $(1,0,0)$ \\ 
      \hline

  %\bottomrule
  \hline
  \end{tabular}
  }
}
\end{table}

==> tables/tbl-instruction-part3.tex <==
\begin{table}
\centering
\small
  \mycaption{tab:exp-4p3}
{Results of \textit{Experiment-4 Part 3}.}
{\textit{$(x, y, z)$: $x$ true positives, $y$ false positives, and $z$ false negatives.)}
}
{
\resizebox{\columnwidth}{!}{
  \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
          \backslashbox{Ask}{Actual}
      & \textbf{Event} & \textbf{Check} &  \textbf{Call} & 
                \textbf{Assign} &
                \textbf{Signature} & \textbf{Return}  \\
     \hline
      \textbf{Event}  &  $(2,0,1)$ & $(0,0,3)$  & $(0,0,2)$ & $(0,0,1)$ & $(0,0,3)$ & $(0,0,1)$  \\ 
      \hline 
      \textbf{Check}&  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline
       \textbf{Call} &  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline
       \textbf{Assign} &  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline
      \textbf{Signature} &  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline
      \textbf{Return} &  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline
      \textbf{All} &  $(0,0,0)$ & $(0,0,0)$  & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0)$ & $(0,0,0) $\\                                                        \hline

  %\bottomrule
  \hline
  \end{tabular}
  }
}
\end{table}

==> tables/tbl-large-1.tex <==
\begin{table}[t]
\centering
\small

\mycaption{tab:large}
{Evaluation results on the large dataset.}
{
}
{
%\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{|l|c|c|c|c|c|c||c|c|}
\hline
                 &  \multicolumn{2}{c|}{\textbf{High}} & \multicolumn{2}{c|}{\textbf{Medium}} & \multicolumn{2}{c||}{\textbf{Low}}  & \multicolumn{2}{c|}{{\textbf{Total}}} \\ 

\cline{2-3}
\cline{4-5}
\cline{6-7}
\cline{8-9}

 & {{\textbf{TP}}} &  {{\textbf{FP}}}  & {{\textbf{TP}}} &  {{\textbf{FP}}}  & {{\textbf{TP}}} &  {{\textbf{FP}}} & {{\textbf{TP}}} &  {{\textbf{FP}}} \\

\hline
\hline

{\textbf{ERC20}}     & 1 & 0 & 95 & 0  & 24  & 4   & 120  & 4    \\ \hline
{\textbf{ERC721}}    & 0 & 1 & 3  & 3  & 107 & 1   & 110 & 5  \\ \hline
{\textbf{ERC1155}}   & 3 & 0 & 12 & 0  & 25  & 1   & 40  & 1 \\ \hline \hline
{\textbf{Total}}     & 4 & 1 & 110 & 3  & 156 & 6   & 270 & 10 \\ \hline

\end{tabular}
%}
}

% \vspace{-0.2in}
\end{table}

==> tables/tbl-realworld.tex <==


\begin{table}[h]

    \centering
    \begin{tabularx}{\columnwidth}{lXX|XXX}
    \hline
    \multirow{2}{*}{\textbf{Contracts}} & \multirow{2}{*}{\textbf{TP}} & \multirow{2}{*}{\textbf{FP}} & \multicolumn{3}{c}{\textbf{Violation Severity}} \\
    \cline{4-6}
    & & & \textbf{High} & \textbf{Medium} & \textbf{Low} \\
    \hline
    100 ERC20 & 79 & 10 & 1 & 55 & 23 \\
    \hline
    50 ERC721 & 109 & 9 & 0 & 3 & 106 \\
    \hline
    50 ERC1155 & 34 & 1 & 1 & 15 & 18 \\
    \hline

    \end{tabularx}
    \caption{200 Most Recent Smart Contracts Auditing Result}
    \label{tab:token_type_analysis}
\end{table}

==> tables/tbl-requirement.tex <==
\begin{table}
\centering
\small
  \mycaption{tab:exp-1}
{Results of \textit{Experiment-1}.}
{\textit{(C: contract code, TTF: token-transfer function, 
CR: contract requirements, and FR: function requirements.
$(x, y, z)$: $x$ true positives, $y$ false positives, and $z$ false negatives.)}
}
{
  \begin{tabular}{|l|c|c|c|c|c|}
    %\toprule
    \hline
            % \multicolumn{2}{c}{Full Contract} & \multicolumn{3}{c}{Token-Transfer Function} \\ 
        %\cmidrule(lr){2-3}
        %\cmidrule(lr){4-6}
                & \textbf{C+CR} & \textbf{C} &  \textbf{TTF+CR} & \textbf{TTF} & \textbf{TTF+FR} \\
     %      \midrule
     \hline

      ERC20  &  $(0,0,2)$ & $(0,0,2)$  & $(3,0,0)$ & $(3,0,0)$  &  $(3,0,0)$    \\ \hline 
      ERC721 & $(0,0,0)$ & $(0,0,0)$ & $(0,0,3)$ & $(3,0,0)$ & $(3,0,0)$ \\                                                        \hline
      ERC777 & $(0,0,0)$ & $(0,0,0)$ & $(0,0,3)$ & $(3,0,0)$ & $(3,0,0)$ \\                                                        \hline

      
  %\bottomrule
  \hline
  \end{tabular}
}
\end{table}



==> tables/vio_inj_table.tex <==
\begin{table}[h]
\begin{tabular}{|c|c|}
\hline
\textbf{Violation Root Causes} & \textbf{ Method } \\
\hline
Missing action - Incorrect action & No action \\
\hline
Missing action - Incorrect action & Another action \\
\hline
Missing action - Incorrect parameter(s) & Wrong order \\
\hline
Missing action - Incorrect parameter(s) & Wrong value \\
\hline
Missing action - Incorrect condition(s) & No condition(s) \\
\hline
Missing action - Incorrect condition(s) & Wrap action with if(false){ ... } \\
\hline
Missing action - Incorrect condition(s) & condition(s) \&\& false != false \\
\hline
Missing action - Incorrect condition(s) & condition(s) \&\& true != true \\
\hline
Missing action - Incorrect condition(s) & !condition(s)  \\
\hline
Missing action - Incorrect condition(s) & Wrap action with while(false){ ... }  \\
\hline
Missing action - Incorrect condition(s) & conditions(s) \&\& (true != true || 1 != 1)  \\
\hline
\end{tabular}

\caption{Violation Injection Table}
\label{tab:vio-inj}

\end{table}
